Domain Wall Constraints on Two Higgs Doublet Models with $Z_2$ Symmetry

The Two Higgs Doublet Model (2HDM) with spontaneously broken $Z_2$ symmetry predicts a production of domain walls at the electroweak scale. We derive cosmological constraints on model parameters for both Type-I and Type-II 2HDMs from the requirement that domain walls do not dominate the Universe by the present day. For Type-I 2HDMs, we deduce the lower bound on the key parameter $\tan\beta > 10^5$ for a wide range of Higgs-boson masses $\sim$ 100 GeV or greater close to the Standard Model alignment limit. In addition, we perform numerical simulations of the 2HDM with an approximate as well as an exact $Z_2$ symmetry but biased initial conditions. In both cases, we find that domain wall networks are unstable and, hence, do not survive at late times. The domain walls experience an exponential suppression of scaling in these models which can help ameliorate the stringent constraints found in the case of an exact discrete symmetry. For a 2HDM with softly-broken $Z_2$ symmetry, we relate the size of this exponential suppression to the soft-breaking bilinear parameter $m_{12}$ allowing limits to be placed on this parameter of order $\mu$eV, such that domain wall domination can be avoided. In particular, for Type-II 2HDMs, we obtain a corresponding lower limit on the CP-odd phase $\theta$ generated by QCD instantons, $\theta \ \stackrel{>}{{}_\sim}\ 10^{-11}/(\sin\beta \cos\beta)$, which is in some tension with the upper limit of $\theta \ \stackrel{<}{{}_\sim}\ 10^{-11}$--$10^{-10}$, as derived from the non-observation of a non-zero neutron electric dipole moment. For a $Z_2$-symmetric 2HDM with biased initial conditions, we are able to relate the size of the exponential suppression to a biasing parameter $\varepsilon$ so as to avoid domain wall domination.

==> Sections/Phenomenology/Phenomenology.tex <==
\section{Particle Physics Phenomenology}
\label{sec:ppPhenom}

The fermions and electroweak gauge bosons of the SM acquire their masses via their coupling to the Higgs field.
In other words, the SM VEV, $v_\text{SM}$, appears in the quadratic mass terms for the fermions and electroweak gauge bosons in the Yukawa and gauge-kinetic terms of the SM Lagrangian, respectively.
In the $Z_2$-symmetric 2HDM the VEVs of the two Higgs doublets, as well as the SM VEV itself, change in the vicinity of a domain wall as the solution interpolates from one vacuum to another as illustrated in Fig.~\ref{fig:Z2vac_kink}.
In either vacuum with SM alignment, particle interactions will be the same as those predicted in the SM, nontheless, the masses and interactions of fundamental particles in the 2HDM will vary locally around domain walls of the type shown in Fig.~\ref{fig:Z2vac_kink}.
In this section, we consider what effect a 2HDM domain wall would have on the masses and interactions of SM particles.
{\bf Discuss the charge-breaking walls from the simulations paper.}
Particular attention will be given to the effects on the photon.
Using the general parametrization of the vacua, we obtain the gauge masses and interactions from the kinetic term of the Lagrangian,
\begin{equation}
    \mathcal{L}_\text{kin} = \left|D_\mu\Phi_1\right|^2 + \left|D_\mu\Phi_2\right|^2,
\end{equation}
where the gauge-covariant derivative can be written as
\begin{equation}
    D_\mu = \left(\begin{matrix}
    \partial_\mu + \frac{i}{2}(gW_\mu^3 + g^\prime B_\mu) & \frac{ig}{2}(W_\mu^1 - iW_\mu^2) \\
    \frac{ig}{2}(W_\mu^1 + iW_\mu^2) & \partial_\mu - \frac{i}{2}(g W_\mu^3 - g^\prime B_\mu)
    \end{matrix}\right).
\end{equation}
For $v_+ = 0$, one obtains the usual expressions for the masses of the electroweak gauge bosons in terms of the model parameters,
\begin{equation}
    M_{W^\pm} = \frac{1}{2} g v_\text{SM}, \quad
    M_{Z^0} = \frac{g v_\text{SM}}{2\cos\theta_W}, \quad
    M_\gamma = 0.
\end{equation}
Where the eletroweak bosons are defined as
\begin{equation}
    W_\mu^{\pm} = \frac{1}{\sqrt{2}}(W_\mu^1 \mp iW_\mu^2)
\end{equation}
and
\begin{equation}
    \left(\begin{matrix}
    Z_\mu \\
    A_\mu
    \end{matrix}\right) = 
    \left(\begin{matrix}
    \cos\theta_W & -\sin\theta_W \\
    \sin\theta_W & \cos\theta_W
    \end{matrix}\right)\left(\begin{matrix}
    W_\mu^3 \\
    B_\mu
    \end{matrix}\right)
\end{equation}
with weak mixing angle, $\tan\theta_W = g^\prime/ g$.
The spatial variation of the electroweak boson mass eigenvalues corresponding to the kink of Fig.~\ref{fig:Z2vac_kink} is illustrated in Fig.~\ref{fig:gauge_mass_nvac}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{Sections/Phenomenology/Images/gauge_masses_0.pdf}
    \caption{Spatial variation of the mass eigenvalues of the electroweak gauge bosons for a neutral vacuum kink solution with parameters $M_H = M_a = M_{H^\pm} = 200$ GeV, $\tan\beta = 0.85$, $\cos(\alpha - \beta) = 1.0$, $g = 0.65$ and $\theta_W = 0.5$ rad.}
    \label{fig:gauge_mass_nvac}
\end{figure}
As expected, in either of the degenerate vacua, the electroweak boson masses are those of the SM, however, the masses decrease locally in the vicinity of a 2HDM domain wall where $v_\text{SM}$ changes value.
%{\color{red} Derive the gauge-Higgs interaction matrix.}
One can similarly derive expressions for the mass of the fermions by expanding the Yukawa lagrangian.
The masses and interactions of particles in either domain will be unaffected, nonetheless, the physics will change locally on a domain wall.

For solutions of the type found in our simulations where there is a local violation of the neutral vacuum condition \cite{Viatic2020} and, hence, a non-zero $v_+$, the mass matrix for the gauge bosons becomes more complicated:
\begin{equation}
    \small
   \mathcal{M}_\text{EW}^2 = \frac{g^2}{4} \left(
\begin{array}{cccc}
  v_1^2+v_2^2+v_+^2 & 0 & 0 & 2 v_2 v_+ c_\xi \tan \theta_W \\
 0 & v_1^2+v_2^2+v_+^2 & 0 & 2 v_2 v_+ s_\xi \tan \theta_W \\
 0 & 0 & v_1^2+v_2^2+v_+^2 &  -\left(v_1^2+v_2^2-v_+^2\right) \tan \theta_W \\
 2 v_2 v_+ c_\xi \tan \theta_W & 2 v_2 v_+ s_\xi \tan \theta_W &  -\left(v_1^2+v_2^2-v_+^2\right) \tan \theta_W &  \left(v_1^2+v_2^2+v_+^2\right) \tan^2 \theta_W \\
\end{array}
\right).
\end{equation}
The masses of the $W^\pm$ bosons are unchanged, however, the photon, $\gamma$, acquires a mass $v_+ \ne 0$ and the $Z^0$ boson mass is also modified:
\begin{equation}\label{eq:photonmass}
    \begin{split}
    M_\gamma^2 & = \frac{g^2 \left(v_1^2+v_2^2+v_+^2 -\sqrt{(v_1^2+v_2^2+v_+^2)^2 - 4\sin^2(2\theta_W)v_1^2v_+^2}\right)}{8\cos^2\theta_W} \\
    & = \frac{g^2 \left(2R^0 -\sqrt{(2R^0)^2  - 4\sin^2(2\theta_W) R_\mu R^\mu}\right)}{8\cos^2\theta_W}
    \end{split}
\end{equation}
and
\begin{equation}
    \begin{split}
    M_Z^2 & = \frac{g^2 \left(v_1^2+v_2^2+v_+^2 + \sqrt{(v_1^2+v_2^2+v_+^2)^2 - 4\sin^2(2\theta_W)v_1^2v_+^2}\right)}{8\cos^2\theta_W} \\
    & = \frac{g^2 \left(2R^0 + \sqrt{(2R^0)^2 - 4\sin^2(2\theta_W) R_\mu R^\mu}\right)}{8\cos^2\theta_W}.
    \end{split}
\end{equation}
%Note that we have made use of \eqref{eq:RVectorVac} to express the mass eigenvalues in terms of the components of $R^\mu$.
The vacuum manifold parameter, $v_+$, is locally non-zero in the vicinity of our domain wall solutions but is zero in either vacuum.
Therefore, the photon is predicted to acquire a mass locally in the vicinity of a 2HDM domain wall of the type found in our simulations.
The spatial variation of the gauge boson masses for an example kink solution are given in Fig.~\ref{fig:gauge_mass_cvac}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{Sections/Phenomenology/Images/gauge_masses_1.pdf}
    \caption{Spatial variation of electroweak gauge bosons mass eigenvalues for a kink solution with non-zero $v_+$, i.e. a relative electroweak rotation between vacua. Parameters chosen were $M_H = M_a = M_{H^\pm} = 200$ GeV, $\tan\beta = 0.85$, $\cos(\alpha - \beta) = 1.0$, $g = 0.65$ and $\theta_W = 0.5$ rad.}
    \label{fig:gauge_mass_cvac}
\end{figure}
We again find a local variation in the mass of the electroweak gauge bosons, however, in this case we also observe a local variation of the photon mass near the 2HDM domain walls.
Specifically, the photon acquires a mass due to the presence of $v_+$ as predicted by \eqref{eq:photonmass}.
% {\bf Preliminary plot of the photon mass in terms of model parameters in Fig.~\ref{fig:photonmass_var}.}
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{Sections/Phenomenology/Images/photon_var.pdf}
%     \caption{{\bf Variation of photon mass as function of physical parameters in SM alignment for solutions with relative electroweak rotation between vacua as in sims. paper.}}
%     \label{fig:photonmass_var}
% \end{figure}

To further investigate this phenomenon, we now consider the phenomenology of photon-domain wall interactions.
Let us linearize the Higgs doublets and electroweak gauge fields, $B_\mu$ and $\mathbf{W}_\mu \equiv W_\mu^a \frac{\sigma^a}{2}$, in one dimension as
\begin{equation}
    \Phi_i(x,t) = \Phi_i^0(x) + \delta \Phi_i(x,t), \quad B_\mu = B_\mu^0 + \delta B_\mu, \quad \mathbf{W}_\mu = \mathbf{W}_\mu^0 + \delta \mathbf{W}_\mu
\end{equation}
where $\Phi_i^0(x)$ is a background kink profile.
The equations of motion for these fields can be derived to be
\begin{equation}\label{eq:ScalarEoM}
    D_\mu D^\mu \Phi_i + \frac{\partial V}{\partial \Phi_i^\dagger} = 0,
\end{equation}
\begin{equation}\label{eq:U1EoM}
    \partial_\mu B^{\mu\nu} = \frac{i g^\prime}{2}\left[\Phi_i^\dagger D^\nu \Phi_i - (D^\nu\Phi_i)^\dagger \Phi_i\right]
\end{equation}
and
\begin{equation}\label{eq:SU2EoM}
    \partial_\mu W^{\mu\nu\,a} + g\varepsilon^{abc}W_\mu^b W^{\mu\nu,c} = \frac{ig}{2}\left[\Phi_i^\dagger\sigma^a D^\nu\Phi_i^\dagger - \left(D^\nu\Phi_i\right)^\dagger\sigma^a\Phi_i\right]
\end{equation}
where summation over repeated indices is implied.
The tensors
\begin{equation}
    W_{\mu\nu}^a = \partial_\mu W_\nu^a - \partial_\nu W_\mu^a - g \varepsilon^{abc} W_\mu^b W_\nu^c
\end{equation}
and
\begin{equation}
    B_{\mu\nu} = \partial_\mu B_\nu - \partial_\nu B_\mu
\end{equation}
are the $\text{SU}(2)_L$ and $\text{U}(1)_Y$ field strengths, respectively.
The gauge-covariant derivative is given by
\begin{equation}
    D_\mu = \partial_\mu + \frac{ig}{2} W_\mu^a \sigma^a + \frac{i g^\prime}{2}B_\mu.
\end{equation}
where $\sigma^a$ are the Pauli matrices.
{\bf Linearize these EoMs in 1D with a simulation-type kink background in unitary gauge.}
